Improving Sequential Recommenders through Counterfactual Augmentation of System Exposure

In sequential recommendation (SR), system exposure refers to items that are exposed to the user. Typically, only a few of the exposed items would be interacted with by the user. Although SR has achieved great success in predicting future user interests, existing SR methods still fail to fully exploit system exposure data. Most methods only model items that have been interacted with, while the large volume of exposed but non-interacted items is overlooked. Even methods that consider the whole system exposure typically train the recommender using only the logged historical system exposure, without exploring unseen user interests. In this paper, we propose counterfactual augmentation over system exposure for sequential recommendation (CaseRec). To better model historical system exposure, CaseRec introduces reinforcement learning to account for different exposure rewards. CaseRec uses a decision transformer-based sequential model to take an exposure sequence as input and assigns different rewards according to the user feedback. To further explore unseen user interests, CaseRec proposes to perform counterfactual augmentation, where exposed original items are replaced with counterfactual items. Then, a transformer-based user simulator is proposed to predict the user feedback reward for the augmented items. Augmentation, together with the user simulator, constructs counterfactual exposure sequences to uncover new user interests. Finally, CaseRec jointly uses the logged exposure sequences with the counterfactual exposure sequences to train a decision transformer-based sequential model for generating recommendation. Experiments on three real-world benchmarks show the effectiveness of CaseRec. Our code is available at https://github.com/ZiqiZhao1/CaseRec.

==> sections/8_acknowledgements.tex <==
\section{Acknowledgements}

